Dynamic balancing of planar mechanisms using toric geometry

In this paper, a new method to determine the complete set of dynamically balanced planar four-bar mechanims is presented. Using complex variables to model the kinematics of the mechanism, the dynamic balancing constraints are written as algebraic equations over complex variables and joint angular velocities. After elimination of the joint angular velocity variables, the problem is formulated as a problem of factorization of Laurent polynomials. Using toric polynomial division, necessary and sufficient conditions for dynamic balancing of planar four-bar mechanisms are derived.

==> figure/NewtonPolygonsCoeff.latex <==
\setlength{\unitlength}{4144sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(2806,2806)(398,-2814)
\thinlines
{\color[rgb]{0,0,0}\put(1801,-961){\line(-1, 0){450}}
}%
{\color[rgb]{0,0,0}\put(1801,-961){\line( 1,-1){450}}
}%
{\color[rgb]{0,0,0}\put(2251,-1411){\line( 0,-1){405}}
}%
{\color[rgb]{0,0,0}\put(2251,-1816){\line(-1, 0){450}}
}%
{\color[rgb]{0,0,0}\put(1801,-1816){\line(-1, 1){450}}
}%
{\color[rgb]{0,0,0}\put(1351,-1456){\line( 0, 1){495}}
}%
{\color[rgb]{0,0,0}\put(451,-2761){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(901,-2761){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(1351,-2761){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(1801,-2761){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(2251,-2761){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(2701,-2761){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(3151,-2761){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(451,-2311){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(901,-2311){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(1351,-2311){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(1801,-2311){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(2251,-2311){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(2701,-2311){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(3151,-2311){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(451,-1816){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(901,-1816){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(1351,-1816){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(1801,-1816){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(2251,-1816){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(2701,-1816){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(3151,-1816){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(451,-1411){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(901,-1411){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(1351,-1411){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(1801,-1411){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(2251,-1411){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(2701,-1411){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(3151,-1411){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(451,-961){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(901,-961){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(1351,-961){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(1801,-961){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(2251,-961){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(2701,-961){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(3151,-961){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(451,-511){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(901,-511){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(1351,-511){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(1801,-511){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(2251,-511){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(2701,-511){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(3151,-511){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(901,-61){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(1351,-61){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(1801,-61){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(2251,-61){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(2701,-61){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(3151,-61){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(1351,-1816){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(901,-961){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(901,-511){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(1351,-511){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(1351,-1411){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(1351,-961){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(1801,-961){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(1801,-1411){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(1801,-1816){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(2251,-2311){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(2251,-1816){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(2251,-1411){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(2251,-961){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(2701,-2311){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(2701,-1816){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(451,-61){\circle{90}}
}%
{\color[rgb]{0,0,0}\put(901,-961){\line( 0, 1){450}}
\put(901,-511){\line( 1, 0){450}}
\put(1351,-511){\line( 5,-3){880.147}}
\put(2251,-1006){\line( 3,-5){476.471}}
\put(2701,-1816){\line( 0,-1){495}}
\put(2701,-2311){\line(-1, 0){450}}
\put(2251,-2311){\line(-5, 3){880.147}}
\put(1351,-1816){\line(-1, 2){432}}
}%
\put(2206,-826){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}A1}%
}}}}
\put(721,-421){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}B1}%
}}}}
\put(631,-1096){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}C1}%
}}}}
\put(1306,-421){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}D1}%
}}}}
\put(1216,-826){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}E1}%
}}}}
\put(1666,-871){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}F1}%
}}}}
\put(2161,-1321){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}G1}%
}}}}
\put(1216,-2041){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}A2}%
}}}}
\put(2656,-2536){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}B2}%
}}}}
\put(2746,-1726){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}C2}%
}}}}
\put(2116,-2536){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}D2}%
}}}}
\put(2206,-2041){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}E2}%
}}}}
\put(1801,-1996){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}F2}%
}}}}
\put(1261,-1591){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}G2}%
}}}}
\put(1666,-1321){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}H}%
}}}}
\end{picture}%

